Cut-Toggling and Cycle-Toggling for Electrical Flow and Other p-Norm Flows

We study the problem of finding flows in undirected graphs so as to minimize the weighted $p$-norm of the flow for any $p > 1$. When $p=2$, the problem is that of finding an electrical flow, and its dual is equivalent to solving a Laplacian linear system. The case $p = \infty$ corresponds to finding a min-congestion flow, which is equivalent to max-flows. A typical algorithmic construction for such problems considers vertex potentials corresponding to the flow conservation constraints, and has two simple types of update steps: cycle toggling, which modifies the flow along a cycle, and cut toggling, which modifies all potentials on one side of a cut. Both types of steps are typically performed relative to a spanning tree $T$; then the cycle is a fundamental cycle of $T$, and the cut is a fundamental cut of $T$. In this paper, we show that these simple steps can be used to give a novel efficient implementation for the $p = 2$ case and to find near-optimal $p$-norm flows in a low number of iterations for all values of $p > 1$. Compared to known faster algorithms for these problems, our algorithms are simpler, more combinatorial, and also expose several underlying connections between these algorithms and dynamic graph data structures that have not been formalized previously.

==> conclusion.tex <==

\section{Conclusion} \label{sec:conclusion}
We propose a cut-based combinatorial algorithm to solve Laplacian systems approximately. This algorithm is dual to the cycle-based algorithm by Kelner et al. \cite{KOSZ13}. We show that our algorithm converges in a near-linear number of iterations. 

\todo{mention that lower bound isn't an impossibility proof?}
\todo{is the data structure hardness vs. runtime bound due to offline vs. online, or due to a different notion of approximation?}

To achieve a near-linear running time, we would further need each iteration to run in polylogarithmic time. We give evidence against this, by presenting a reduction from the OMv conjecture. This is in contrast to the algorithm in \cite{KOSZ13}, which uses a data structure such that each iteration of the algorithm runs in $O(\log n)$ time.   In order to obtain a better running time, one would need to  show it is possible take advantage of the particular structure of updates in the algorithm to implement the data structure.  Note that our reduction crucially needs that a very specific spanning tree (albeit with very small stretch) is chosen. Is it possible for the algorithm to choose a different small-stretch spanning tree that is amendable to a polylogarithmic time implementation?
%performs $O(n)$ updates followed by $O(n)$ executions of \textsf{findflow}, whereas our algorithm only needs to alternate between \textsf{addvalue} and \textsf{findflow}.  Possibly this structure is amendable to a polylogarithmic time implementation?

% \section{Todo}
% \textbf{Things to do in terms of research:}
% \begin{enumerate}
%     \item Bound the overall running time of this algorithm. (See Section 4.3).
% \end{enumerate}

% \textbf{Things to do in terms of writing:}
% \begin{enumerate}
%     \item Instead of setting $R(C) = \sum_{(k, l) \in \delta(C)} \frac{1}{r(k, l)}$, set
%     $R(C) = \left(\sum_{(k, l) \in \delta(C)} \frac{1}{r(k, l)}\right)^{-1}$. This way, $R(C)$ has the units of resistance instead of units of $\mathrm{resistance}^{-1}$, which makes more sense. 
%     \item Make notation more consistent, and clearer. For example, $\Delta(C)$ or $\Delta(C(i, j))$ or $\Delta(C(i, j), p)$? Also tree-defined flow is currently denoted $\mathbf{f_T}$, whereas the potential-defined flow is denoted $\mathbf{f}$, which is kind of confusing. 
% \end{enumerate}
